CAMP: Compiler and Allocator-based Heap Memory Protection

The heap is a critical and widely used component of many applications. Due to its dynamic nature, combined with the complexity of heap management algorithms, it is also a frequent target for security exploits. To enhance the heap's security, various heap protection techniques have been introduced, but they either introduce significant runtime overhead or have limited protection. We present CAMP, a new sanitizer for detecting and capturing heap memory corruption. CAMP leverages a compiler and a customized memory allocator. The compiler adds boundary-checking and escape-tracking instructions to the target program, while the memory allocator tracks memory ranges, coordinates with the instrumentation, and neutralizes dangling pointers. With the novel error detection scheme, CAMP enables various compiler optimization strategies and thus eliminates redundant and unnecessary check instrumentation. This design minimizes runtime overhead without sacrificing security guarantees. Our evaluation and comparison of CAMP with existing tools, using both real-world applications and SPEC CPU benchmarks, show that it provides even better heap corruption detection capability with lower runtime overhead.

==> sections/4_design.tex <==
\section{Design}
\subsection{Approach Overview}
CAMP is an efficient memory protection mechanism that can make memory corruption vulnerabilities unexploitable. If we can prevent memory corruption at the root cause code, the attacker will not be able to exploit the vulnerabilities. 

The root cause of out-of-bound bugs is wrong pointer creation or calculation.  When there is a memory overflow that happens from one memory chunk to another memory chunk (either it is linear or non-linear), there always has a memory reference computation that changes the memory reference from one chunk to another chunk. Our detection of out-of-bound is based on this observation. To do the detection, we insert codes using the compiler to track all the memory pointer computation, once there is a computation causing a cross chunk of the reference, we report the out-of-bound. 

The root cause of use-after-free is program failed to clean up freed memory reference in time. In CAMP, some codes are inserted to keep track of memory allocation and reference.  The tracked memory references let us know where they are and we could simply patch the reference to the memory being freed to a non-canonical address to prevent UAF.

\subsection{Memory Allocator and Runtime}
\subsection{Compilation Optimization}
% To prevent UAF, 

To prevent OOB, CAMP instruments every pointer calculation operation and pointer type conversion operation with a check function. Each check will query the lower bound and 
upper bound of the corresponded chunk and check whether the pointer in the range of chunk.

\subsubsection{Merging Similar Checks}

The first technique aims to merge similar checks, two checks are considered similar when the two pointers being checked can be calculated by the same pointer. Here is an example of similar checks:

\begin{lstlisting}[language=C++, caption=Similar Checks Example]
@ \textcolor{red}{check(flag, 0)} @
 flag[0] = 0;
@ \textcolor{red}{check(flag, 1)} @
 flag[1] = 0;
 for(int i = 2; i < n; ++i){
     @\textcolor{red}{check(flag, i)} @
     if (flag[i]){
         for(int j = i*i; j < n; j += i){
             @\textcolor{red}{check(flag, j)} @
             flag[j] = 0;
         }
     }
 }
\end{lstlisting}

Note that even though these checks are used to check different pointers, all pointers are calculated from the same base pointer. Specifically, all checked pointers in the code snippet are calculated from \texttt{flag}, it means that all pointers should in the same chunk and are constrained by the same upper and lower bounds. Considering each check need to find the range of chunk that the base pointer represented first so that we only need to query the chunk range once in a very first place, then every checks can use the result of the query to check whether the pointer in the correct range. The operation will be very cheap, because it only requires two comparison operations with the lower bound and upper bound of the chunk but no more memory read/write operations. We call such optimization \textit{Merging Similar Checks}. 

\paragraph{Merging Similar Checks}
Formally, given two pointer \texttt{ptr1} and \texttt{ptr2}, \texttt{check(ptr1)} and \texttt{check(ptr2)} can be merge if \texttt{base(ptr1)= base(ptr2)}. \texttt{base(p)} gets the base address of the object that \texttt{p} points to.

To implement the optimization, we use an intra-procedural analysis to locate the base pointers for every pointers that need to be checked. In LLVM IR, \texttt{getelementptr} instructions and \texttt{bitcast} instructions are used for pointer calculation, so these instructions need to be checked. The \texttt{getelementptr} instruction contains a pointer operand and many offset operands, and the result pointer of \texttt{getelementptr} instruction is derived from the pointer operand. The \texttt{bitcast} instruction is used to convert the type of pointer, it only contains only one pointer operand so that the result pointer of \texttt{bitcast} is derived from the pointer operand. We will backward trace the propagation of the pointer until an instruction that is neither \texttt{getelementptr} nor \texttt{bitcast}. We assume the instruction's result is the base pointer of original pointer.

This optimization reveals the greater optimization space of our design compared to ASAN. There has been a lot of previous work trying to optimize ASAN, including trying to merge check operations. However, these works require more requirements for mergeable checks. It means that less code can be optimized.  Considering that most code will use a pointer more than once,  this optimization will work in almost every function that has pointer operations. \textcolor{red}{May be we need a table to support it.} On the other hand, although our single check costs larger than ASAN, our design allows this cost to be spread evenly over multiple checks, so our overall overhead will be better than ASAN.

\subsubsection{Optimizing Structure Checks}

The second technique aims to optimize the checks for inflexible structure-type pointers. We claim that every \texttt{getelementptr} that act on inflexible structure type pointers do not need to be checked in runtime. Although intuitively the statement is not correct, we will prove it is right in our framework in the following paragraph.

The structure type pointer optimization relies on two key features. The first feature is that the offset operands of 
\texttt{getelementptr} instruction that act on inflexible structure type pointer
is always constant in LLVM IR. \textcolor{red}{I am not sure how to prove it more strictly} Hence, if the size of chunk pointed by a structure type pointer is larger than the size of the structure type can be guaranteed in runtime, all \texttt{getelementptr} instructions that act on inflexible structure type pointer will not overflow. The property can be guaranteed by the second feature.

The second feature is LLVM type system is a strong type system, it implies that every type conversions must be explicit in LLVM IR. Although C and C++ support implicit type conversion, LLVM IR will still insert explicit type conversion instructions. The following code is an example:

Considering that the return type of general allocation function (see Table \ref{tab:alloc}) is \texttt{void*} or \texttt{i8*} in LLVM IR and every objects on the heap area are created by dynamic allocation function, so that structure type pointer cannot be created by allocation function directly but with at least one more explicit type conversion instruction. Note that we have added checks for all type conversion instruction (\texttt{bitcast} instruction) so that the size of the chunk that is pointed by a structure type pointer in the program is always larger than the size of the structure type or CAMP will detect it and stop the program. 

This optimization are also effective and can extremely reduce the overhead of runtime. Nowdays most large software often contain hundreds of or even thousands of different stucture type, most large software today often contains hundreds or even thousands of different structure types, and programs access these structures very frequently. This optimization can avoid to check this structure type pointer calculation.

\begin{table}
    \centering
    \begin{tabular}{c|c}
        \hline
            Lang & Function \\ \hline
        \multirow{7}*{\texttt{C} } 
              & \texttt{\small void* malloc(size\_t)} \\
            ~ & \texttt{\small void* calloc(size\_t, size\_t)}  \\
            ~ & \texttt{\small void* realloc(void *, size\_t)} \\
            ~ & \texttt{\small void* memalign(size\_t)} \\
            ~ & \texttt{\small void *valloc(size\_t size)} \\
            ~ & \texttt{\small void *pvalloc(size\_t size)} \\
            ~ & \texttt{\small int posix\_memalign(void**, size\_t, size\_t)} \\
        \hline
        \multirow{4}*{\texttt{C++} } 
              & \texttt{\small void* operator new(size\_t)} \\
            ~ & \texttt{\small void* operator new[](size\_t)} \\
            ~ & \texttt{\small void* operator new(size\_t, align\_val\_t)} \\
            ~ & \texttt{\small void* operator new[](size\_t, align\_val\_t)} \\
        \hline
    \end{tabular}
    \caption{Memory Allocation Function Prototype}
    \label{tab:alloc}
\end{table}

\subsubsection{Other Common Optimization}
The above two optimizations are customized for our designs. To further reduce overhead of CAMP, we also deployed some common optimization techniques.

\paragraph{Simplify Range Query} If a pointer calculation and allocation operation are in the same scope, we can directly fetch the return value and parameters of the call to memory allocation function as the base pointer and pointer's size. We call such query method builtin query. In almost all scenarios, builtin queries are much faster than queries in runtime. 
\paragraph{Removing Unsatisfiable Checks} If we can confirm at compile time that a certain pointer calculation must not produce an illegitimate pointer, then we can remove the check for this pointer calculation. For example, a \texttt{bitcast} instruction converts a pointer's type into another type which size is smaller or the offset of one pointer is always less than the size of the pointer. 

\paragraph{Removing Redundant Checks}
If one pointer calculation instruction dominates or post-dominates another one and the first instruction's pointer range larger than the second instruction's pointer range, the checks for the second instruction are considered redundant and could be eliminated. 

